CHOrD: Generation of Collision-Free, House-Scale, and Organized Digital Twins for 3D Indoor Scenes with Controllable Floor Plans and Optimal Layouts

We introduce CHOrD, a novel framework for scalable synthesis of 3D indoor scenes, designed to create house-scale, collision-free, and hierarchically structured indoor digital twins. In contrast to existing methods that directly synthesize the scene layout as a scene graph or object list, CHOrD incorporates a 2D image-based intermediate layout representation, enabling effective prevention of collision artifacts by successfully capturing them as out-of-distribution (OOD) scenarios during generation. Furthermore, unlike existing methods, CHOrD is capable of generating scene layouts that adhere to complex floor plans with multi-modal controls, enabling the creation of coherent, house-wide layouts robust to both geometric and semantic variations in room structures. Additionally, we propose a novel dataset with expanded coverage of household items and room configurations, as well as significantly improved data quality. CHOrD demonstrates state-of-the-art performance on both the 3D-FRONT and our proposed datasets, delivering photorealistic, spatially coherent indoor scene synthesis adaptable to arbitrary floor plan variations.

==> TODO.tex <==
While converting the bounding box sizes to absolute units, we examine the wall thickness in the image





LLMs can generate layouts, but scaling up is difficult, and they cannot prevent collisions due to their limited spatial understanding. Additionally, it is nontrivial to train LLMs to generate layouts with a distribution close to real datasets.

We anticipate a series of intriguing applications of \ourmethod{} in a variety of applications such as simulated training and testing for embodied AI, interior design, and virtual and augmented reality.

==> images/floor_text_2_layout.tex <==
\begin{figure}
% \vspace{-6mm}
\centering
\begin{subfigure}{0.46\linewidth}
    \includegraphics[width=\linewidth]{images/floor2layout.png}
    \caption{Floor plan to layout generation. }
    \label{fig:floor2layout}
\end{subfigure}
\begin{subfigure}{0.46\linewidth}
    \includegraphics[width=\linewidth]{images/text2layout.png}
    \caption{Text description to layout generation}
    \label{fig:text2layout}
\end{subfigure}  
\caption{Two types of layout generation proposed in \ourmethod{}}
\vspace{-5mm}
\label{fig:cam_compare}
\end{figure}

==> pdfs/ablation.tex <==
\begin{figure}
    \centering
    % 第一组
    \begin{tabular}{ccc}
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/grays/gray__1_.png}
        \end{subfigure} &
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/grays/gray__2_.png}
        \end{subfigure} &
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/grays/gray__3_.png}
        \end{subfigure} \\
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/grays/color__1_.png}
        \end{subfigure} &
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/grays/color__2_.png}
        \end{subfigure} &
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/grays/color__3_.png}
        \end{subfigure} \\
        % \multicolumn{3}{c}{\small} \\
    \end{tabular}
    
    \hrule % 分割线
    
    % 第二组
    \vspace{0.5em} % 增加分割线和组之间的间距
    \begin{tabular}{ccc}
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/grays/gray__4_.png}
        \end{subfigure} &
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/grays/gray__5_.png}
        \end{subfigure} &
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/grays/gray__6_.png}
        \end{subfigure} \\
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/grays/color__4_.png}
        \end{subfigure} &
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/grays/color__5_.png}
        \end{subfigure} &
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/grays/color__6_.png}
        \end{subfigure} \\
        % \multicolumn{3}{c}{\small} \\
    \end{tabular}
    
    \hrule % 分割线
    
    % 第三组
    \vspace{0.5em} % 增加分割线和组之间的间距
    \begin{tabular}{ccc}
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/grays/gray__7_.png}
        \end{subfigure} &
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/grays/gray__8_.png}
        \end{subfigure} &
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/grays/gray__9_.png}
        \end{subfigure} \\
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/grays/color__7_.png}
        \end{subfigure} &
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/grays/color__8_.png}
        \end{subfigure} &
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/grays/color__9_.png}
        \end{subfigure} \\
        % \multicolumn{3}{c}{\small} \\
    \end{tabular}
    
    \caption{\modify{Visualization of ablation study results. Grayscale images represent segmentation maps directly generated by the diffusion model. Each segmentation map is converted into an RGB-based layout image, consistent with the color scheme described in Table~\ref{tab:furniture}. While inaccuracies in the grayscale images are not directly observed due to insufficient precision, the converted color images clearly reveal that the generated segmentation maps contain significantly more artifacts compared to the layouts generated by \ourmethod{}.}}
    \label{fig:ablation}
\end{figure}

==> sections/Statements.tex <==
\section{Ethics Statement}

In this work, we adhere to responsible research practices, ensuring that the datasets and methods used comply with legal and ethical standards. The dataset created and utilized in this study was sourced and generated without infringing on the rights of individuals or organizations. We have ensured that the data is free of personally identifiable information, and that no harm has been inflicted on any subjects during the research process. Furthermore, the research addresses technical challenges in generative indoor scene synthesis, with no direct societal or environmental risks.

\section{Reproducibility Statement}

To ensure the reproducibility of our work, we have provided the source code in the supplementary materials, along with detailed descriptions of our methodology and experimental setup in the main paper. The \ourmethod{} model, including hyperparameters, training procedures, and evaluation metrics, has been thoroughly documented. Upon acceptance, we will publicly release the source code, pretrained models, and our novel \ourdataset{} to facilitate verification and further research in this field.
